When Should an Agent Refresh? Adaptive Index Reuse for Efficient Long-Horizon Reasoning

Language agents read code, tool output, and dialogue in contexts that grow at every step. Dynamic sparse attention lets a small indexer choose the earlier tokens each query attends to, but the indexer still scores the whole prefix at every layer. Cross-layer reuse methods such as IndexCache rerun the indexer at only some layers, with one fixed pattern for every input. In an agent, the relevant evidence can change abruptly when a traceback or test result arrives, so fresh selections matter more at some steps than at others. We propose Adaptive Index Reuse (AIR), which keeps IndexCache's execution and learns, for each segment of an agent episode, how many layers refresh their selection. A small controller reads signals from completed computation and the latest tool event, chooses a pattern from a nested library, and learns from terminal task reward under an expected compute budget. On Qwen3-4B-Instruct-2507 with a 128K context, AIR improves success over the strongest static schedule at matched cost on SWE-bench Verified (27.0% to 32.4%), Terminal-Bench 2.0, and three $\tau^2$-bench domains, and it lowers time per successful task on all five. Across 50 backbone, context, and benchmark settings, it matches or exceeds that schedule in 44.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> results/cases/case_retail_part1.tex <==
\caseheading{A policy restriction can make extra refresh unnecessary}{Does increasing refresh after a policy observation help when every method can already apply the restriction?}
\begin{rolebox}[title={Shared initial task}]{taskpurple}
I would like to return the headphones in order R-order because they do not fit comfortably. The customer and visible order state are identical across branches.
\end{rolebox}
\begin{rolebox}[title={Event 1: Read the order}]{toolslate}
\smalllabel{Available before decision.} The customer supplies the order identifier and asks to return the headphones because they do not fit comfortably.
\end{rolebox}
\begin{tcbraster}[raster columns=2,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{get\_order}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=5$; causal event features. Prefix after call: 1,198 tokens.\par Selections: 5,990; key updates: 43,128.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{get\_order}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,198 tokens.\par Selections: 10,782; key updates: 10,782.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The order record marks the headphones as opened and final sale. The applicable return rule has not yet been retrieved.}\par
\begin{rolebox}[title={Event 2: Check the applicable rule}]{toolslate}
\smalllabel{Available before decision.} The completed order lookup identifies opened, final-sale headphones. Eligibility still requires the applicable rule.
\end{rolebox}
\begin{tcbraster}[raster columns=2,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{get\_return\_rules}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; causal event features. Prefix after call: 1,734 tokens.\par Selections: 10,814; key updates: 62,424.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{get\_return\_rules}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,728 tokens.\par Selections: 15,552; key updates: 15,552.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The returned rule states that opened final-sale headphones are ineligible for a comfort-related return.}\par


==> results/cases/case_retail_part2.tex <==
\caseheading{A policy restriction can make extra refresh unnecessary (continued)}{Event 3 and the end state}
\begin{rolebox}[title={Event 3: Reconcile the order facts}]{toolslate}
\smalllabel{Available before decision.} The restriction is now visible. It is a completed observation before the next budget choice.
\end{rolebox}
\begin{tcbraster}[raster columns=2,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{get\_order}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=18$; causal event features. Prefix after call: 2,092 tokens.\par Selections: 17,258; key updates: 75,312.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{get\_order}\par \texttt{order\_id="R-order"}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 2,084 tokens.\par Selections: 18,756; key updates: 18,756.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The order facts remain unchanged; the restriction applies to this request.}\par
\begin{rolebox}[title={Visible final messages}]{agentblue}
\textbf{AIR.} ``The return rule excludes opened final-sale headphones for this reason, so I cannot request this return.'' \textbf{Fixed IndexCache R9.} ``The return rule excludes opened final-sale headphones for this reason, so I cannot request this return.''
\end{rolebox}
\begin{rolebox}[title={End state and interpretation}]{authoramber}
\textbf{AIR.} No unsupported return is requested; the restriction is explained. \textbf{Fixed IndexCache R9.} The same policy-compliant end state is reached.\par Both methods reach the same policy-compliant end state. AIR makes fewer Full-layer selections but maintains more index keys, so the two counters move in opposite directions and neither alone gives the total cost.
\end{rolebox}
{\figfont AIR maintains all 36 eligible-layer keys.}


==> results/cases/case_swe_part1.tex <==
\caseheading{A new diagnostic changes the allocation question}{When should a new visible test diagnostic trigger a higher refresh budget?}
\begin{rolebox}[title={Shared initial task}]{taskpurple}
Repair the date-range helper so an equal start and end date is retained. Inspect the existing boundary tests and add a focused regression test. The same working tree and task text are presented to every method.
\end{rolebox}
\begin{rolebox}[title={Event 1: Inspect the boundary}]{toolslate}
\smalllabel{Available before decision.} The task reports an equal-boundary defect. The relevant repository content is available only through the read tool.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=10}\par \texttt{end=40}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=5$; causal event features. Prefix after call: 1,368 tokens.\par Selections: 6,840; key updates: 49,248.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=10}\par \texttt{end=40}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,368 tokens.\par Selections: 12,312; key updates: 12,312.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={ReTopK (indexer-adapted)}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=10}\par \texttt{end=40}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Exact tool-output prefill; decode-selection reuse. Prefix after call: 1,368 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The function uses a strict comparison; the visible neighboring tests identify tests/test\_ranges.py.}\par
\begin{rolebox}[title={Event 2: Edit and request a check}]{toolslate}
\smalllabel{Available before decision.} The completed read identifies the boundary comparison. The edit and test request below follow this observation.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{apply\_patch}\\Boundary patch: change \texttt{start < end} to \texttt{start <= end}.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; causal event features. Prefix after call: 1,840 tokens.\par Selections: 11,088; key updates: 66,240.}}\endgroup\par\vspace{4pt}\texttt{run\_tests}\par \texttt{command="python -m pytest tests/test\_ranges.py"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=3$; causal event features. Prefix after call: 2,090 tokens.\par Selections: 11,838; key updates: 75,240.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{apply\_patch}\\Boundary patch: change \texttt{start < end} to \texttt{start <= end}.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,840 tokens.\par Selections: 16,560; key updates: 16,560.}}\endgroup\par\vspace{4pt}\texttt{run\_tests}\par \texttt{command="python -m pytest tests/test\_ranges.py"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 2,090 tokens.\par Selections: 18,810; key updates: 18,810.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={ReTopK (indexer-adapted)}]{agentblue}
\texttt{apply\_patch}\\Boundary patch: change \texttt{start < end} to \texttt{start <= end}.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Exact tool-output prefill; decode-selection reuse. Prefix after call: 1,840 tokens.}}\endgroup\par\vspace{4pt}\texttt{run\_tests}\par \texttt{command="python -m pytest tests/test\_ranges.py"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Exact tool-output prefill; decode-selection reuse. Prefix after call: 2,090 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The test response reports a reversed-range diagnostic that was not available before the test request.}\par


==> results/cases/case_swe_part2.tex <==
\caseheading{A new diagnostic changes the allocation question (continued)}{Event 3 and the end state}
\begin{rolebox}[title={Event 3: Read the newly relevant branch}]{toolslate}
\smalllabel{Available before decision.} The returned test diagnostic includes a traceback/test-result flag about the reversed-range branch.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=35}\par \texttt{end=65}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=18$; causal event features. Prefix after call: 2,706 tokens.\par Selections: 22,926; key updates: 97,416.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=35}\par \texttt{end=65}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 2,712 tokens.\par Selections: 24,408; key updates: 24,408.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={ReTopK (indexer-adapted)}]{agentblue}
\texttt{read\_file}\par \texttt{path="range\_utils.py"}\par \texttt{start=35}\par \texttt{end=65}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Exact tool-output prefill; decode-selection reuse. Prefix after call: 2,710 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The read exposes the newly relevant branch and the code that needs a follow-up revision.}\par
\begin{rolebox}[title={End state and interpretation}]{authoramber}
\textbf{AIR.} The newly relevant branch is identified for a follow-up revision. \textbf{Fixed IndexCache R9.} The same branch is identified with a constant budget. \textbf{ReTopK (indexer-adapted).} The same branch is identified under exact tool-output prefill and decode reuse.\par AIR raises its refresh budget at the model call after the test diagnostic appears, while fixed IndexCache keeps R=9 and ReTopK reuses decode selections. All methods identify the same next repair step, so the case shows when each spends index work.
\end{rolebox}
{\figfont AIR maintains all 36 eligible-layer keys.}


==> results/cases/case_terminal_part1.tex <==
\caseheading{Long output does not imply expensive work forever}{Can allocation fall after the useful part of a long command output has been isolated?}
\begin{rolebox}[title={Shared initial task}]{taskpurple}
Build the local wheel into dist/ and confirm that the expected entry point is present in its metadata. All branches begin in the same project directory with the same shell tools. The expected console-script entry is example-cli = example\_pkg.cli:main.
\end{rolebox}
\begin{rolebox}[title={Event 1: Inspect the environment}]{toolslate}
\smalllabel{Available before decision.} The task names the output directory and expected entry point. The working directory has not yet been inspected.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{shell}\par \texttt{command="pwd \&\& ls"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=5$; causal event features. Prefix after call: 1,620 tokens.\par Selections: 8,100; key updates: 58,320.}}\endgroup\par\vspace{4pt}\texttt{shell}\par \texttt{command="python -m build --wheel --outdir dist"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=5$; causal event features. Prefix after call: 1,894 tokens.\par Selections: 9,470; key updates: 68,184.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{shell}\par \texttt{command="pwd \&\& ls"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,620 tokens.\par Selections: 14,580; key updates: 14,580.}}\endgroup\par\vspace{4pt}\texttt{shell}\par \texttt{command="python -m build --wheel --outdir dist"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 1,894 tokens.\par Selections: 17,046; key updates: 17,046.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={HISA + static R9}]{agentblue}
\texttt{shell}\par \texttt{command="pwd \&\& ls"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Static $R=9$; hierarchical selector. Prefix after call: 1,620 tokens.}}\endgroup\par\vspace{4pt}\texttt{shell}\par \texttt{command="python -m build --wheel --outdir dist"}\par \texttt{timeout\_s=120}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Static $R=9$; hierarchical selector. Prefix after call: 1,894 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The build report names dist/example\_pkg-0.1-py3-none-any.whl, includes extensive dependency output and flags a changed build-environment setting.}\par
\begin{rolebox}[title={Event 2: Read a lengthy build report}]{toolslate}
\smalllabel{Available before decision.} The completed build report contains a changed environment setting among the long output.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{shell}\par \texttt{command="cat pyproject.toml"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=18$; causal event features. Prefix after call: 4,084 tokens.\par Selections: 48,890; key updates: 147,024.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{shell}\par \texttt{command="cat pyproject.toml"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 4,084 tokens.\par Selections: 36,756; key updates: 36,756.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={HISA + static R9}]{agentblue}
\texttt{shell}\par \texttt{command="cat pyproject.toml"}\par \texttt{timeout\_s=30}\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Static $R=9$; hierarchical selector. Prefix after call: 4,082 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The configuration identifies the expected console-script target; the relevant setting is now isolated.}\par


==> results/cases/case_terminal_part2.tex <==
\caseheading{Long output does not imply expensive work forever (continued)}{Event 3 and the end state}
\begin{rolebox}[title={Event 3: Inspect a focused output}]{toolslate}
\smalllabel{Available before decision.} The wheel path and expected entry point are known from completed observations.
\end{rolebox}
\begin{tcbraster}[raster columns=3,raster equal height=rows,raster valign=top,raster column skip=3pt,raster before skip=0pt,raster after skip=1pt]
\begin{rolebox}[title={AIR}]{agentblue}
\texttt{shell}\par Read entry\_points.txt from the named wheel with Python zipfile.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=3$; causal event features. Prefix after call: 4,386 tokens.\par Selections: 49,796; key updates: 157,896.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={Fixed IndexCache R9}]{agentblue}
\texttt{shell}\par Read entry\_points.txt from the named wheel with Python zipfile.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par $R=9$; fixed mask. Prefix after call: 4,386 tokens.\par Selections: 39,474; key updates: 39,474.}}\endgroup
\end{rolebox}
\begin{rolebox}[title={HISA + static R9}]{agentblue}
\texttt{shell}\par Read entry\_points.txt from the named wheel with Python zipfile.\par\vspace{2pt}\begingroup\setlength{\fboxsep}{2.5pt}\colorbox{controlteal!8}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{\raggedright\figfont \smalllabel{Controller / selector}\par Static $R=9$; hierarchical selector. Prefix after call: 4,384 tokens.}}\endgroup
\end{rolebox}
\end{tcbraster}
{\figfont\smalllabel{Returned after the action.} The metadata text contains example-cli = example\_pkg.cli:main, matching the requested entry-point mapping.}\par
\begin{rolebox}[title={End state and interpretation}]{authoramber}
\textbf{AIR.} The requested metadata inspection is completed. \textbf{Fixed IndexCache R9.} The same metadata inspection is completed. \textbf{HISA + static R9.} The same metadata inspection is completed; hierarchical selector work needs its own accounting.\par AIR spends more refresh when a long command output arrives and less once the relevant lines are isolated, and the early extra work can outweigh the later savings. HISA latency and the end-to-end ranking also depend on hierarchical selector work, which the Full-layer counter leaves out.
\end{rolebox}
{\figfont AIR maintains all 36 eligible-layer keys.}


==> results/cases/controller_telemetry_contract.tex <==
\caseheading{Controller telemetry and operation counts}{Causal observations remain separate from the agent prompt}
\begin{rolebox}[title={Read before the action}]{controlteal}
The default controller reads position, observed environment events and accumulated cost, together with lagged model and index summaries from completed computation. The first segment marks lagged values as missing. Hidden tests, future tool responses, terminal reward and repository identity are excluded. The controller runs outside the agent's prompt and conversation.\par
Every new model invocation starts a decision segment. An additional boundary occurs after each 512 decoded tokens. Every decode span in this gallery is shorter than 512 tokens, so the next shown decision is at the next invocation. All branches use the same primary-model menu: $R\in\{3,5,9,18,36\}$.
\end{rolebox}
\begin{rolebox}[title={Masks and caches}]{controlteal}
The first eligible layer is always Full. A Full layer writes selected position IDs for the current query; a Shared layer uses the nearest preceding Full layer's IDs and its own KV tensors. Selected-ID buffers reset for every query. Native noneligible layers neither read nor overwrite these buffers. AIR maintains index keys at all 36 eligible layers.\par
The nested mask order used in these cases starts with layers $\{1,7,24\}$ and adds layers 13 and 32 at $R=5$. The $R=9$ mask adds 4, 11, 19 and 35. Appendix~\ref{app:library} describes how the trained libraries are built.
\end{rolebox}
\begin{rolebox}[title={Exactly what the counts mean}]{toolslate}
For a listed invocation, let $q=q_{\rm prefill}+q_{\rm decode}$. The flat indexer performs $qR$ Full-layer selection calls. AIR performs $36q$ index-key updates; the specialized fixed-$R9$ implementation performs $9q$. The panels report cumulative sums of these counts. Prefix length is the cumulative prefill and decode-token count in each branch.\par
No paid probe appears here. The counters stop at the last listed tool-producing invocation and exclude generation of the visible final prose messages. They also omit controller arithmetic, attention, non-index model work, tool time and environment time. They therefore measure index work only, which is part of complete episode cost and elapsed time. ReTopK and HISA perform different selector operations, so their counts are kept separate from the flat-indexer counter.
\end{rolebox}
\begin{rolebox}[title={An example counter identity}]{authoramber}
The first SWE invocation has 1,280 prefill queries and 88 decode queries: $q=1,368$. AIR at $R=5$ performs 6,840 Full-layer selections and 49,248 key updates. Fixed $R9$ performs 12,312 selections and 12,312 key updates. Because the counters cover index work only, their difference is not a speedup.
\end{rolebox}


